VITA: Video Instance Segmentation via Object Token Association

We introduce a novel paradigm for offline Video Instance Segmentation (VIS), based on the hypothesis that explicit object-oriented information can be a strong clue for understanding the context of the entire sequence. To this end, we propose VITA, a simple structure built on top of an off-the-shelf Transformer-based image instance segmentation model. Specifically, we use an image object detector as a means of distilling object-specific contexts into object tokens. VITA accomplishes video-level understanding by associating frame-level object tokens without using spatio-temporal backbone features. By effectively building relationships between objects using the condensed information, VITA achieves the state-of-the-art on VIS benchmarks with a ResNet-50 backbone: 49.8 AP, 45.7 AP on YouTube-VIS 2019 & 2021, and 19.6 AP on OVIS. Moreover, thanks to its object token-based structure that is disjoint from the backbone features, VITA shows several practical advantages that previous offline VIS methods have not explored - handling long and high-resolution videos with a common GPU, and freezing a frame-level detector trained on image domain. Code is available at https://github.com/sukjunhwang/VITA.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} We describe the limitations of our work as a future research direction in \cref{sec:conclusion}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} We included potential misuses in Broader Impact.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerNA{}
  \item Did you include complete proofs of all theoretical results?
     \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} We listed the data and instructions in \cref{sec:experiments} and Appendix, and the code will be released upon acceptance.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} We specified details in \cref{sec:impl_details}.
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} We reported error bars and score of five runs in \cref{sec:experiments}.
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} We included the type of resources used for training and inference in Appendix.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} We cited the papers and repositories that are used.
  \item Did you mention the license of the assets?
    \answerYes{} We mentioned the license at the end.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{} New assets are not included.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{} Not the scope of this paper.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{} Not the scope of this paper.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{} Not the scope of this paper.
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tab/disjoint.tex <==
\begin{table}
\centering
\caption{
% 
Per-frame pretrain.
% 
} % \caption
\resizebox{\linewidth}{!}
{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}c|c|c|c|c|c|ccccc@{}}
\toprule
Backbone    & Image         & Video         & Num Frames    & Resolution    & Max Mem   & AP    & AP$_{50}$ & AP$_{75}$ & AR$_{1}$  & AR$_{10}$ \\
\midrule
\midrule
ResNet-50   &               & \checkmark    & 6             & Low           & 28.8 G    \\
ResNet-101  &               & \checkmark    & 6             & Low           & \\
\midrule
ResNet-50   & \checkmark    & \checkmark    & 6             & Low           & \\
ResNet-101  & \checkmark    & \checkmark    & 6             & Low           & \\
Swin-L      & \checkmark    & \checkmark    & 6             & Low           & \\
\midrule
ResNet-50   & \checkmark    & \checkmark    & 18            & Low           & \\
ResNet-101  & \checkmark    & \checkmark    & 18            & Low           & \\
Swin-L      & \checkmark    & \checkmark    & 18            & Low           & \\
\midrule
ResNet-50   & \checkmark    & \checkmark    & 6             & High          & \\
ResNet-101  & \checkmark    & \checkmark    & 6             & High          & \\
Swin-L      & \checkmark    & \checkmark    & 6             & High          & \\
\bottomrule
\end{tabular}
} %< \resizebox
\label{tab:disjoint}
\end{table}

==> tab/pruning.tex <==
\begin{table}
\centering
\caption{
% 
Pruning tokens by different ratios.
% 
} % \caption
% \resizebox{\linewidth}{!}
{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}l|ccccc@{}}
\toprule
$r$         & AP    & AP$_{50}$ & AP$_{75}$ & AR$_{1}$  & AR$_{10}$ \\
\midrule
\midrule
1.0         & 49.8  & 72.6      & 54.5      & 49.4      & 61.0      \\
0.75        & 49.7  & 72.5      & 54.4      & 48.7      & 61.0      \\
0.5         & 48.9  & 72.1      & 52.0      & 48.3      & 60.9      \\
0.25        & 48.1  & 71.6      & 51.6      & 47.4      & 59.8      \\
\bottomrule
\end{tabular}
} %< \resizebox
\label{tab:pruning}
\end{table}

==> tab/swin_ytvis2021.tex <==
\begin{table}
\centering
\caption{
% 
Comparisons on YouTube-VIS 2021.
% 
} % \caption
%\resizebox{\linewidth}{!}
{ %< auto-adjusts font size to fill line
\begin{tabular}{l|l|ccccc}
    \toprule
    Method                                  & Backbone~\cite{Swin}              & AP        & AP$_{50}$ & AP$_{75}$ & AR$_1$    & AR$_{10}$ \\
    \midrule
    \midrule
    SeqFormer~\cite{SeqFormer}                                                  & Swin-L                    & 51.8      & 74.6      & 58.2      & 42.8      & 58.1      \\
    Mask2Former-VIS~\cite{Mask2Former-VIS}                                      & Swin-L                    & 52.6      & 76.4      & 57.2      & -         & -         \\
    \midrule
    \textbf{VITA (Ours)}                    & \textbf{Swin-L}           & \textbf{57.5}      & \textbf{80.6}      & \textbf{61.0}      & \textbf{47.7}      & \textbf{62.6}      \\
    \bottomrule
    \end{tabular}
} %< \resizebox
\label{tab:swin_ytvis21}
%\vspace{-5mm}
\end{table}
